Spatially Multi-conditional Image Generation

In most scenarios, conditional image generation can be thought of as an inversion of the image understanding process. Since generic image understanding involves solving multiple tasks, it is natural to aim at generating images via multi-conditioning. However, multi-conditional image generation is a very challenging problem due to the heterogeneity and the sparsity of the (in practice) available conditioning labels. In this work, we propose a novel neural architecture to address the problem of heterogeneity and sparsity of the spatially multi-conditional labels. Our choice of spatial conditioning, such as by semantics and depth, is driven by the promise it holds for better control of the image generation process. The proposed method uses a transformer-like architecture operating pixel-wise, which receives the available labels as input tokens to merge them in a learned homogeneous space of labels. The merged labels are then used for image generation via conditional generative adversarial training. In this process, the sparsity of the labels is handled by simply dropping the input tokens corresponding to the missing labels at the desired locations, thanks to the proposed pixel-wise operating architecture. Our experiments on three benchmark datasets demonstrate the clear superiority of our method over the state-of-the-art and compared baselines. The source code will be made publicly available.

==> figures/paper/taskonomy.tex <==
%\addtolength{\tabcolsep}{-3.5pt}  
\begin{figure*}[b]
\centering
\begin{tabular} {cc|cc|cc}
 Labels & Ground Truth & SPADE~\cite{park2019semantic} & ASAP~\cite{RottShaham2020ASAP} & TLAM~ & Sparse TLAM \\
 
\includegraphics[width=2.6cm]{images/paper/taskonomy/168-all-crop.pdf}& 
 \includegraphics[width=2.6cm]{images/paper/taskonomy/point_168_view_2_domain_rgb_gt.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_168_view_2_domain_rgb_spade.png} &   \includegraphics[width=2.6cm]{images/paper/taskonomy/point_168_view_2_domain_rgb_asap.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_168_view_2_domain_rgb_all.png} &  \includegraphics[width=2.6cm]{images/paper/taskonomy/point_168_view_2_domain_rgb_sparse.png} \\

& \includegraphics[width=2.6cm]{images/paper/taskonomy/point_296_view_2_domain_rgb_gt.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_296_view_2_domain_rgb_spade.png} &   \includegraphics[width=2.6cm]{images/paper/taskonomy/point_296_view_2_domain_rgb_asap.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_296_view_2_domain_rgb_all.png} &  \includegraphics[width=2.6cm]{images/paper/taskonomy/point_296_view_2_domain_rgb_sparse.png} \\

& \includegraphics[width=2.6cm]{images/paper/taskonomy/point_817_view_3_domain_rgb_gt.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_817_view_3_domain_rgb_spade.png} &   \includegraphics[width=2.6cm]{images/paper/taskonomy/point_817_view_3_domain_rgb_asap.png} &
\includegraphics[width=2.6cm]{images/paper/taskonomy/point_817_view_3_domain_rgb_all.png} &  \includegraphics[width=2.6cm]{images/paper/taskonomy/point_817_view_3_domain_rgb_sparse.png} \\

\end{tabular}
	\caption{Visual comparison on the Taskonomy datasets. Our methods is able to generate more realistic images with fine details.}
	\label{fig::taskonomy}
\end{figure*}


==> latex_submission/paper/method_old.tex <==
\section{Method}

%for structured data: use $\mathsf{X}$: matrix/tensor
%for unstructured data: use $\mathcal{X}$: sets

We start by introducing a few formal notations. As an input, we have a collection of labels $\mathcal{X}=\{\mathsf{X_1}, \mathsf{X_2}, ..., \mathsf{X_N}\}$, where each label $\mathsf{X_k} \in \mathbb{R}^{H \times W \times C_k}$ has height $H$, width $W$ and $C_k$  channels. The element of the label $\mathsf{X_k}$ corresponding to height $i$ and width $j$ is denoted as $\mathsf{x_{k}^{ij}} \in \mathbb{R}^{C_k}$. Also, elements of the label collection $\mathcal{X}$ corresponding to height $i$ and width $j$ form a collection $\mathcal{X}^{ij}=\{\mathsf{x_{1}^{ij}}, \mathsf{x_{2}^{ij}}, ..., \mathsf{x_{N}^{ij}}\}$. The model takes the collection of labels $\mathcal{X}$ as an input and produces $\mathsf{O} = N (\mathcal{X})$, where $\mathsf{O} \in \mathbb{R}^{H \times W \times 3}$ is the generated image.

\subsection{Network Overview}
\label{sec:network_overwiev}
The proposed model is divided into two components: the label merging component and the image generation component. This is depicted in Figure~\ref{fig:main_teaser}. 

The first model component is the label merging. It takes the collection of labels $\mathcal{X}$ as the input and merges them into $\mathsf{Z} = M(\mathcal{X})$, where $\mathsf{Z} \in \mathbb{R}^{H \times W \times d}$ is the \emph{Concept Tensor}. It is interesting to note that the label merging block does not require the number of input labels to be the same for every input. Input labels $\mathcal{X}$ are heterogeneous because different labels $\mathsf{X_k}$ come from different sources and they can have different numbers of input channels $C_k$, as well as different ranges of values. For example, semantic segmentation labels are one way of describing a certain image understanding aspect through discrete values, while surface normals are one way of describing certain geometric properties of the scene through continuous values. Therefore, the job of the label merging block is to first translate all the provided input labels $\mathsf{X_k}$ into the same language, by projecting them into a homogeneous latent space. Then,  all the necessary information that these labels provide is extracted and merged. In short, the label merging block fuses the heterogeneous collection of input labels $\mathcal{X}$ into a homogeneous Concept Tensor $\mathsf{Z}$. This block is depicted in Figure~\ref{fig:LAME_block}.

The second model component is the image generation. It takes the produced Concept Tensor $\mathsf{Z}$ as the input and produces the generated image $\mathsf{O} = G(\mathsf{Z}) = G(M(\mathcal{X})) = N(\mathcal{X})$. The job of the generator is to use all the available information of the input labels $\mathcal{X}$, provided through the homogeneous embedding $\mathsf{Z}$, to generate the desired image $\mathsf{O}$.

\subsection{Label Merging}
We start by describing the mechanics of the label merging component, as illustrated in Figure~\ref{fig:LAME_block}. This component will process different spatial locations of the input labels $\mathcal{X}^{ij}$ independently. We empirically found this to be sufficient. To this end, we first collapse the spatial dimensions of every label $\mathsf{X_k}$ to obtain $\mathsf{\bar{X}_k} \in \mathbb{R}^{HW \times C_k}$, which contains $H\!\cdot\!W$ token vectors $\mathsf{\bar{x}_{k}^{i}} \in \mathbb{R}^{C_k}$ of dimension $C_k$.
The label merging is performed by two blocks: the projection block and the concept generation block, which we described in the following.

\subsubsection{Projection Block}
\label{sec:projection_block}
This block projects every heterogeneous input label $\mathsf{\bar{X}_k}$ into a homogeneous embedding space $\mathsf{\mathsf{\Tilde{X}_k}} \in \mathbb{R}^{HW \times d}$, where $d$ is the dimensionality of the embedding space.
It does so by transforming every token $\mathsf{\bar{x}_{k}^{i}}$ with the projection function $f_k$, which projects it into a homogeneous embedding space $\mathsf{\Tilde{x}_{k}^{i}} = f_k (\mathsf{\bar{x}^{i}})$, where $\mathsf{\Tilde{x}_{k}^{i}} \in \mathbb{R}^{d} $. Every input label shares the same projection function $f_k$ for all tokens, but different input labels $\mathsf{\bar{X}_k}$ have different projection functions $f_k$. We use an affine transformation followed by the GeLU nonlinearity $a(\cdot)$~\cite{hendrycks2020GELU} to serve as the embedding function
\begin{equation}
    \label{eq:projection_block}
    \mathsf{\Tilde{x}_{k}^{i}} = f_k (\mathsf{\bar{x}_{k}^{i}}) = a(\mathsf{A_{k}}\mathsf{\bar{x}_{k}^{i}} + b_k),
\end{equation}
where $\mathsf{A_k} \in \mathbb{R}^{d \times C_k }$ and $\mathsf{b_k} \in \mathbb{R}^{d}$. We implement this by using fully connected layers as projection functions for each input label $\mathsf{\bar{X}_k}$, followed by the GeLU activation function.  Our method also works with sparse input labels, which can be caused by label definition or missing labels. When the value of a label $\mathsf{X_k}$ is missing at a certain spatial location, its corresponding token $\bar{x}_{k}^{i}$ is set to a zero vector. Thus, a token with the embedding $\mathsf{\Tilde{x}_{k}^{i}} = a(b_k)$ will send a signal to the concept generation block that label $k$ is not present at this location, and that it should extract the information from other labels which are present. Also the absence of the whole label $\mathsf{\bar{X}_k}$ is handled in the same manner, by setting all of its tokens to zero vectors.

\subsubsection{Concept Generation Block}
\label{ssec:concept_generation}
The collection of all embedded tokens from the spatial location $i$, $\mathcal{\Tilde{X}}^{i} = \{ \mathsf{\Tilde{x}_{1}^{i}}, \mathsf{\Tilde{x}_{2}^{i}}, ..., \mathsf{\Tilde{x}_{N}^{i}} \}$, is now processed by the concept generation block.

\noindent\textbf{Transformer Label Merging block (TLAM).} This block is build in the spirit of the transformer architecture~\cite{Vaswani2017, dosovitskiy2020vit} and shared across for all spatial locations. Transformers are naturally suited here to encourage interaction between the embedded tokens to share their label specific information while merging it into the final label representation. Before giving $\mathcal{\Tilde{X}}^{i}$ to the transformer, we add label specific encodings $\mathsf{p_k}$ \PR{where do they come from?} to the embedded task tokens $\mathsf{\Tilde{x}_{k}^{i}}$ to obtain $\mathsf{\Tilde{z}_{k}^{i(0)}} = \mathsf{\Tilde{x}_{k}^{i}} + \mathsf{p_k}$. Then we pass $\mathcal{\Tilde{Z}}^{i(0)} = \{ \mathsf{\Tilde{z}_{1}^{i(0)}}, \mathsf{\Tilde{z}_{2}^{i(0)}}, ... , \mathsf{\Tilde{z}_{N}^{i(0)}} \}$ through $l$ consecutive transformer blocks $\mathsf{B}_m$. Each block $\mathsf{B}_m$ takes the output of the previous block $\mathcal{\Tilde{Z}}^{i(m-1)}$ as its input and produces $\mathcal{\Tilde{Z}}^{i(m)}= \mathsf{B}_m(\mathcal{\Tilde{Z}}^{i(m-1)})$, where $\mathcal{\Tilde{Z}}^{i(m)} = \{ \mathsf{\Tilde{z}_{1}^{i(m)}}, \mathsf{\Tilde{z}_{2}^{i(m)}}, ... , \mathsf{\Tilde{z}_{N}^{i(m)}} \}$ and $\mathsf{\Tilde{z}_{k}^{i(m)}} \in \mathbb{R}^{d}$. 

Each transformer block $\mathsf{B}_m$ is composed of a Multi-head Self Attention block (MSA), followed by a Multilayer Perceptron block (MLP)~\cite{Vaswani2017, dosovitskiy2020vit}.
Self-attention is a global operation, where every token interacts with every other token and thus information is shared across them.
Multiple heads in the MSA block are used for more efficient computation and for extracting richer and more diverse features.
The MSA block executes the following operations:
\begin{equation}
    \label{eq:MSA}
    \mathcal{\hat{Z}}^{i(m)} = 
    \mathsf{MSA}(\mathsf{LN}(\mathcal{\Tilde{Z}}^{i(m-1)})) + 
    \mathcal{\Tilde{Z}}^{i(m-1)},
\end{equation}
where $\mathsf{LN}$ represents a Layer Normalization layer~\cite{ba2016LayerNorm}.
The MSA block is followed by the MLP block, which processes each token separately using the same Multilayer Perceptron. 
This block further processes the token features, after their global interactions in the MSA block, by sharing and refining the representations of each token across all their channels. 
The MLP block executes the following operations:
\begin{equation}
    \label{eq:MLP}
    \mathcal{\Tilde{Z}}^{i(m)} = 
    \mathsf{MLP}(\mathsf{LN}(\mathcal{\hat{Z}}^{i(m)})) + 
    \mathcal{\hat{Z}}^{i(m)}.
\end{equation}

Finally, all the elements of the output collection produced by the final transformer block $\mathcal{\Tilde{Z}}^{i(l)} = \{ \mathsf{\Tilde{z}_{1}^{i(l)}}, \mathsf{\Tilde{z}_{2}^{i(l)}}, ... , \mathsf{\Tilde{z}_{N}^{i(l)}} \}$ are averaged to obtain $\mathsf{\Tilde{z}^{i}} = \frac{1}{N} \sum_{k=1:N}\mathsf{\Tilde{z}_{k}^{i}}$. They are reshaped back into the original spatial dimensions to obtain the \emph{Concept Tensor} $\mathsf{Z} \in \mathbb{R}^{H \times W \times d}$. 

\noindent\textbf{Convolutional Label Merging (CLAM).} Additionally, we also explore another simpler way of label merging. Namely, we just stack multiple consecutive blocks similar to the projection block from Section~\ref{sec:projection_block}. The first block is exactly the projection block~\eqref{eq:projection_block}, while the following $l$ blocks perform the same operation with $\mathsf{A}^{l}_k \in \mathbb{R}^{d \times d}, \mathsf{b^{l}_k} \in \mathbb{R}^{d}$, preserving the dimensionality $d$.
After the final block, all output elements corresponding to the same spatial location are averaged to produce the \emph{Concept Tensor} $\mathsf{Z}$, just like at the end of the TLAM block. 

\subsection{Generator}
The task of the generator is to take the produced \emph{Concept Tensor} $\mathsf{Z}$ and to produce the generated image $\mathsf{O} = G(\mathsf{Z})$, as described in Section~\ref{sec:network_overwiev}. As the generator, we employ use the state-of-the-art ASAP model~\cite{RottShaham2020ASAP}. This model first synthesizes the high-resolution pixels using lightweight and highly parallelizable operators. ASAP performs most computationally expensive image analysis at a very coarse resolution. 
We modify the input to ASAP, by providing the \emph{Concept Tensor} $\mathsf{Z}$ as an input, instead of giving only one specific input task $\mathsf{X_k}$. The generator can therefore exploit the merged information from all the available input tasks $\mathcal{X}$.

\begin{comment}
\paragraph{The method continues..}
A recent type of neural network architecture, Transformers, has been proposed in order to handle dynamic information without being tied to a fixed size of the input. Transformers were proposed in the context of natural language processsing. It uses a concept of self-attention matrix in order to dynamically build correlations accorss information in the input. This can be used in out problem setting, where for a particular input only a subset of the information is available, we can adapt the self-attention mechanism. Moreover transformers then allow us to fuse the informations dynamically to provide the best information possible to the generator such that it can convert into an RGB image.



In this work we explore new techniques along the lines of differentiable rendering. Looking at networks like SPADE, they convert a semantic segmentation map into an RGB image. Now the input need not be just a semantic segmentation mask but something more dense like a normal map, depth map etc, which essentially gives more information to the rendering process.

All of these different maps are not readily available in order to differentiably render an image of real world scenarios. Depth maps and others are not easily available for any in the wild image of a scene that we see in the world. However recent method have started exploring the use of convolutional neural networks in order to produce high quality maps from monocular RGB images in the wild. In this work we assume that some of these semantic maps such as surface normals, depth, edges, segmentation and curvature are already available to us. We restrict our problem to the goal of producing a photorealistic RGB image given that these maps are given as input to the network.


An elegant way of mixing information impeding from distinct label is using transformers. A big advantage of transformers are that they can process arbitrary sequence length. Again looking at the usecase of missing label, one can employ this property and drop the missing label from the . We leverage transformer encoder layers on a pixel-level. Each pixel location has multiple label and the self-attention layer in the transformer learns to mix these information. Figure \ref{fig:transformer} shows the composition of this module. In the transformers module each label is first processed individually by MLPs.  Note that the number of MLPs is dependent on the nr of label that are present. This suggests that the network learns the optimal embedding for each label. The MLPs are similar to the ones used in the previous embedding method, except that in this use case the convolutional network is very shallow consisting of only one hidden layer. This preprocessing of the label serves as a first embedding and ensure that all label have the same number of channels before passing to the transformer block. Before  the premilinary embedding of each label can be passed to the transformers block, a positional encoding of each label is required. This helps the Self-Attention block to identify which pixel information belongs to which label. The positional encoding is a parameter that is learned during training and is directly added to the pixel. This idea was proven to be successful in image application of transformers \cite{rw2019timm}.  The transformer block consists of self-attention and feedforward layers and outputs pixelwise feature embedding for each label. These outputs are then averaged to obtain a single feature embedding at every pixel location. The final output of the Module is then a feature embedding of the size $H \times W \times F$, where $H$ and $W$ are the height and width of the full-resolution label maps and $F$ is the channel number of the final embedding. The hyperparameter $F$ is subject to tuning and was set to 96.

When training the network with the Sparse Label input setting the individual label map with the missing pixel information as well as the corresponding mask is taken as input to this transformer module. The sparse label map is treated like in the case of the All Label setting through the transformer networks. Before averaging all the outputs we multiply the corresponding mask to the output tensor. This way the final output tensor carries information on the available and missing pixels.


\end{comment}









==> latex_submission/paper/old_relatedWorks.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Generative Adversarial Networks}
\label{subsec:relgan}
Generative Adversarial Networks \cite{goodfellow2014generative} or  GAN(s) have revolutionised the field of unsupervised deep learning in the recent years. GANs consist of two networks; the generator and the discriminator, which compete with each other in an adversarial training scheme, whose objective is to guide the generator towards learning the distribution of the training data. The generator is expected to learn a function that transforms a sample from a known noise distribution; usually assumed to be the normal distribution, to a corresponding sample from the distribution of the real data; like an image of person's face for example. The job of the discriminator on the other hand is to distinguish samples produced by the generator network from those obtained from the real world training data and flag them as 'fake' samples. The adversarial training of both networks allows the generator to gradually produce samples that resemble the real training data and improve over a period of time as the discriminator gets better a detecting 'fake' samples. This adversarial training, although straightforward in theory, runs into several practical and numerical difficulties, often resulting in the mode collapse of the generator network \cite{thanhtung2020catastrophic}. To circumvent some of these issues, several regularization schemes that prevent the collapse of the generated distribution and increase the stability of training have been proposed \cite{wgan2017, mescheder2018training}.

GANs have been adopted with remarkable success in several domains and have lead to image synthesis with unprecedented realism \cite{karras2018progressive, karras2019stylebased, karras2020analyzing, Karras2021}. In addition to the several regularization schemes mentioned above, a progressive training of the generator and discriminator networks was identified as a key factor in stabilizing high resolution image synthesis \cite{karras2018progressive}. Later, Karras et al. \cite{karras2019stylebased} introduced a style based generative network that proposed a mapping MLP in addition to a modulated convolutional network to allow the generator to disentangle features of the generated image at multiple scales. The quality of the style based generator was further improved in their follow up works, to remove the characteristic artifact \cite{karras2020analyzing} and aliasing effects \cite{Karras2021}. While the work of Karras et al. predominantly concentrated on the architecture and performance of the generator network, Karnewar and Wang \cite{karnewar2020msggan} proposed modifications to the discriminator's architecture to allow for better gradient flow during the backward pass of the generator's training. While it is common for unconstrained generative models to transform a noise sample to a sample of the target distribution, research involving the use of an encoder network to condition the generated sample on a real sample is also gaining momentum \cite{choi2018stargan, choi2020stargan, oord2018neural, razavi2019generating, brock2019large}.  Quite notably, Stargan \cite{choi2018stargan, choi2020stargan} and BigGAN \cite{brock2019large} were able to achieve high quality multi-modal image synthesis with a single class conditioned generative network. Researchers have recently also started to look into normalizing flow networks \cite{Kobyzev_2021} for generative architectures that are invertible \cite{kingma2018glow, styleFlow} and thereby provide additional semantic control at inference time. As generative networks continue to get better, they are increasingly finding use in many practical applications in film and entertainment, medicine, and even games \cite{hao2021GANcraft}. 

\subsection{Image to Image Translation Networks}
\label{subsec:relimg2img}
A special class of deep neural networks that operate on images are \emph{Image to Image Translation} networks. Broadly speaking, these networks often take one or more images as their input and transform them into one or more images at their output. In this area, while Ronneberger et al. originally introduced the \emph{UNet} \cite{ronneberger2015unet} for the task of segmenting medical images, the base architecture itself has been used as a backbone in several important follow up works. \emph{UNets} introduced skip connections between the input and output features of a convolutional neural network to greatly improve gradient flow during training, while also helping preserve the spatial layout of the input in the predicted result. Isola et al. \cite{pix2pix2017} later introduced the \emph{Pix2Pix} paradigm that leveraged the Unet backbone for a generator and combined it with a convolutional discriminator to convert sketches into photo-realistic images. This work was improved upon by Wang et al. to support high resolution image translation in \emph{Pix2PixHD} \cite{wang2018pix2pixHD} and video translation in \emph{Vid2Vid} \cite{wang2018vid2vid}. The improvements suggested by Wang et al. include a modified generator architecture with residual connections \cite{he2015deep} and a patch based discriminator network which can better discern the generated image at multiple scales. They also adopted deep perceptual metrics \cite{simonyan2015deep, zhang2018unreasonable} for supervising the generator instead of the previously used L2 norm. 

Image to image translation networks are immensely useful for several applications in computer vision, including keypoint or landmark detection \cite{newell2016stacked, cao2019openpose, wu2019detectron2}, semantic segmentation \cite{he2018mask, chen2019tensormask, yu2020bisenet}, face reconstruction \cite{sela2017unrestricted, sfsnetSengupta18}, and image based relighting \cite{Sun_2019, Pandey2021} to name a few. As these networks started finding use in several fields, other improvements aimed at reducing their computational burden at inference time were made over time as well. Notable research in this area includes MobileNets \cite{howard2017mobilenets, sandler2019mobilenetv2, howard2019searching} and depthwise separable convolutions \cite{chollet2017xception} which reduce the size of the network and the inference time while sacrificing some performance. Most recently, Shaham et al. introduced the \emph{ASAP-Net} \cite{RottShaham2020ASAP} which achieves the optimal trade off of low inference time, while retaining or even out-performing previous models on several image to image translation tasks. As we employ the \emph{ASAP-Net} as a component in our proposed architecture, we discuss it's structure and working in more details in Chapter.

\subsection{Deep Normalization Techniques}
\label{subsec:relnorm}
There is an increasing desire in the academic and industrial research communities to increase the interpretability of deep neural networks. Understanding the behaviour of deep networks can help us better anticipate and avoid failures, while also providing a window of semantic control. Normalization techniques \cite{dumoulin2018feature-wise, huang2020normalization} are a step in the direction of semantically controllable neural networks with the added benefit of also improving empirical training properties like stability and convergence. In this section, we discuss normalization techniques that have been used in image based networks to instill semantic control over the generated output. Perez et al. introduced a simple  feature-wise linear modulation or FiLM \cite{perez2017film} for the tasking of visual reasoning. Parameters of an affine transformation were derived from a sequence of words, which were then used to explicitly condition the intermediate features of a convolutional network. In the context of neural style transfer \cite{gatys2015neural}, Huang et al. introduced Adaptive Instance Normalization or AdaIn \cite{Huang_2017_ICCV}, wherein the feature-wise statistics from a style image are used to re-normalize the feature space of a content image resulting in the first real time arbitrary style transfer technique. Park et al. extended AdaIN for spatial control in their work SPADE \cite{park2019semantic}, where the normalization parameters are derived from a semantic segmentation image.  SPADE is of particular interest to our work and we elaborate on the details of the method in chapter. Zhu et al. \cite{Zhu_2020_CVPR} further extend SPADE to allow for independent application of global and local style. Finally, generic normalisation schemes that make use of kernel prediction networks to achieve arbitrarily global and local control include Dynamic Instance Normalization (DIN) \cite{jing2019dynamic} and Adaptive Convolutions (AdaConv) \cite{Chandran_2021_CVPR}. While they offer a great deal of flexibility, they also increase the size of the resulting network and sacrifice inference time. 

\subsection{Differentiable Rendering}
\label{subsec:reldiffrender}
In the field of computer graphics, rendering \cite{PBRT3e} refers to the process of converting a 3D scene into an image as seen by a camera, by modelling the physics of light transport. As rendering converts a set of semantically meaningful maps derived from a 3D scene, such as the albedo (shading free color of an object) and the geometry, given a light and a camera, into an image, it can prove to be valuable tool for controllable image generation when combined with neural networks. However, photo-realistic rendering assumes solving the rendering equation which involves recursive evaluations of the incoming and outgoing light at all points on the scene; making its incorporation in the training of a neural network impractical. Furthermore the naturally discontinuous rendering equation, has to made differentiable to allow for bi-directional gradient flow during training. As rendering is a complex and computationally intensive process, several approximations of it have been proposed to facilitate its use for training neural networks. Several methods starting from simple approximations of the rasterization function to produce silhouettes \cite{kato2018renderer, liu2019soft, Laine2020diffrast} to more complex approximations that model indirect lighting effects \cite{Li2018, NimierDavid2020Radiative, Loubet2019Reparameterizing} have been proposed. 
These algorithms have also been incorporated into popular deep learning frameworks such as pytorch \cite{ravi2020pytorch3d, Li2018} and Mitsuba 2 \cite{NimierDavidVicini2019Mitsuba2} to speed up their use in research. Differentiable renderers have been successfully been used in several neural networks including those used for face reconstruction \cite{tewari17MoFA, tewari2018} and human body reconstruction \cite{lin2021endtoend, pavlakos2019expressive} to cite a few. While a thorough review of the techniques and applications of differentiable/neural rendering is beyond the scope of this work, we refer the interested reader to the excellent surveys of Tewari et al. \cite{tewari2020state} and Kato et al. \cite{kato2020differentiable} for more details.

\subsection{Transformers}
\label{subsec:reltransformer}
In the final technical section of the related work, we discuss Transformers and their application in computer vision. Transformers \cite{Vaswani2017} are sequence to sequence networks that were originally proposed for natural language processing. Transformers dynamically build a \emph{self attention} matrix that captures arbitrary correlations between input tokens/elements in a sequence that are arbitrarily far apart and are neural networks that are not tied to operate on a fixed sequence length. Transformers were quickly adopted to process time series and sequential data as they showed remarkable performance benefits over standard recurrent neural networks (RNNs) \cite{schmidt2019recurrent}. Transformers are now the state of the art in language modeling \cite{devlin2019bert, brown2020language} and have even been used to predict complicated protein structures in the breakthrough work \emph{AlphaFold} \cite{AlphaFold2021}. Transformers are finding increasing use in image based networks as well with the introduction of the Vision Transformer \cite{dosovitskiy2020vit} by Dosovitskiy et al.  The vision transformer was quickly leveraged in several follow up works \cite{tolstikhin2021mixer, steiner2021augreg, chen2021outperform, ranftl2021vision} that used Transformers to achieve superior performance on standard image processing tasks like classification and segmentation; fields that have been conventionally dominated by residual convolutional networks \cite{he2015deep}. One of the primary bottlenecks in the training and deployment of a transformer is the quadratic memory complexity in building the attention matrix. The attention matrix is a dense matrix whose dimensions depend on the input/output sequence length of a the transformer. As multiple of these attention matrices are dynamically created during the forward pass of a transformer, GPU memory bottlenecks prevent standard self attention from being used of sequences larger than 512. Linear approximations of the attention matrix such as the Performer \cite{chromanski2021}, Linformer \cite{wang2020linformer}, and the cross-covariance attention (XCA) \cite{el2021} have been proposed recently to allow for longer sequence lengths. Researchers have also started to explore the training of transfomers in unsupervised \cite{caron2021emerging} and adversarial settings \cite{jiang2021transgan}. In this work, we leverage a transformer to address the problem of fusing information from multiple modalities to a common feature space. The details of how we modify the standard transformer to accomplish this is discussed in chapter. 



